The Ghost of Performance Reproducibility Past

The importance of ensemble computing is well established. However, executing ensembles at scale introduces interesting performance fluctuations that have not been well investigated. In this paper, we trace our experience uncovering performance fluctuations of ensemble applications (primarily constituting a workflow of GROMACS tasks), and unsuccessful attempts, so far, at trying to discern the underlying cause(s) of performance fluctuations. Is the failure to discern the causative or contributing factors a failure of capability? Or imagination? Do the fluctuations have their genesis in some inscrutable aspect of the system or software? Does it warrant a fundamental reassessment and rethinking of how we assume and conceptualize performance reproducibility? Answers to these questions are not straightforward, nor are they immediate or obvious. We conclude with a discussion about the performance of ensemble applications and ruminate over the implications for how we define and measure application performance.

==> acknowledgment.tex <==
\section{Acknowledgment}
This work was supported by the U.S. Department of Energy, Office of Science,
Advanced Scientific Computing Research, under Contract DE-AC02-06CH11357. This
research used resources of the Argonne Leadership Computing Facility at
Argonne National Laboratory, which is supported by the Office of Science of
the U.S. Department of Energy under contract DE-AC02-06CH11357.

==> discussion-v2.tex <==
%!TEX root = ./paper.tex

\section{Discussion}
\textcolor{blue} {Although we reduced task runtime variation putatively caused
by OS noise, we still have no good way of \textit{proving} through a set of
measurements that the OS noise was indeed the dominant cause. Employing a
simple metric such as \textit{the number of process context switches} and
directly correlating this measurement to the runtime of a task proved
ineffective in our study because a task affected by OS noise will execute
longer and therefore naturally result in a larger value for this metric. On
the other hand, employing a more sophisticated scheme involving intrusive
instrumentation may affect sensitive applications such as GROMACS and
potentially cause other unintended performance artifacts and overheads that
can obfuscate the behavior being studied. There is a need to fundamentally
understand the genesis of performance variation resulting from exogenous and
endogenous factors and study their impact on critical HPC applications such as
GROMACS. Prior studies have been primarily conducted on (micro)benchmarks ---
it is largely unclear how these results translate to production HPC
applications. We argue that such studies if conducted on upcoming HPC clusters
and made available publicly, would prove helpful to the HPC community at
large, even outside the scope of ensemble computing.}

\textcolor{blue} {Modeling the impact of task level performance variation on HPC ensembles is a challenging endeavor ---
the notion of \textit{performance} now assumes a hierarchical definition. Performance variation observed
at a task level may or may not translate to performance variation at an ensemble workload level, especially
if there are several more tasks to execute than available computing resources. This challenge is conflated with the broader challenge of scheduling the tasks on the available resources. The ability of an ensemble system
to adapt itself based on performance observations of the tasks that have been executed can prove critical to the overall performance of the workflow. In this environment, we view the results of studies from individual applications (such as the one presented here) as tools or knowledge bases for the adaptive system to 
rely on ``if the execution conditions are appropriate''. This view of an adaptive ensemble system implies the existence of (1) a software framework capable of making and actuating these decisions and (2) adaptive policies with specific goals --- performance reproducibility being one of them.
}

Before discussing performance reproducibility in ensemble computations, it is
beneficial to reflect on performance variation assumptions of an HPC
application. It is generally expected that a deterministic application code
will exhibit minor, if any, relevant variation in its performance if it is run
in the same configuration on the same machine. It is this expectation that
forms the basis for HPC performance optimization where inefficiencies can be
reliably identified and improvements made. That said, several exogenous
factors can lead to performance variation, including differences in processor
clock rates, contention with other running codes, operating system
interference, and more. Endogenous to an application, there can be
non-determinism inherent in its execution and fine sensitivities to memory and
network operation.

Nevertheless, it is reasonable to maintain the expectation of
minor performance variation in HPC applications; otherwise, our
performance optimization methodology breaks down. It might be
even assumed possible to characterize any variability within the
context of the application code, in order to determine bounds
and vulnerabilities. With this in mind, performance variation
for an HPC application can be generally regarded as a distribution
around expected performance value, one that very well might be
able to be reproduced. 

However, ensemble execution is a different matter. All factors for performance
variation of a single HPC application are still valid for ensemble tasks.
Instead of a single code, the variability analysis is compounded by the
multiplicity of tasks.
% \jhanote{What are the other sources of ensemble
% performance variability we want to throw out as
% possibilities that are not
% already covered in the exogenous and endogenous
% examples given above? Do we want to talk about tasks
% interfering with other tasks execution/performance?}
Indeed, tasks can interfere with each other as a
result of sharing system infrastructure and cause
perturbations that lead to further performance variation.
In addition, it is essential to realize that how a
task is configured at the time of its execution and the resources assigned are not necessarily fixed.
The same task might be run in a variety of configurations during the lifetime
of the ensemble computation. It is not the optimization of an individual task
under a particular configuration that matters. Task performance naturally has
a much fuller distribution because it covers a potentially broader set of
options that the ensemble runtime system has to choose from during task
scheduling.

A fundamental shift arising from ensemble (task) performance variability is
that it is no longer the performance or optimization of a single task that is
critical, but the collective performance of all ensemble members (viz.,  the
makespan of the workload that matters).
What implications does this have on
performance reproducibility in ensemble computations?  Are we asking for
individual task performance to be reproducible, and by extrapolation, thinking
the ensemble's performance should then be reproducible? Given that an ensemble
workflow maintains task dependencies, does this imply that reproducibility
will require invariance in task execution ordering from one ensemble run to
the next?

% A fundamental implication of ensemble (task) performance variability is that
% it is not the optimization of an individual task under a particular
% configuration that matters.


We contend that the focus of reproducibility should not be on whether an
individual task's performance is reproducible in ensemble computation. When a
task is ready to run, it will then be scheduled and configured according to
the resources allocated. If the task is run again at another point in the
workflow, it might be configured differently and with different resources. It
makes little sense to compare the two task executions if they are configured
differently -- a 4-node MPI+OpenMP task with 32 CPU threads per node will
behave very differently from a 1-process instantiation of the task with 4
GPUs. Here performance variation stares the ensemble scheduler directly in the
face. Furthermore, decisions regarding resource assignment might have less to
do with optimal task performance than with dynamic resource availability and
collective utilization of ensemble resources. Even as we relinquish the belief
of single task performance reproducibility, we are constrained by need for
collective performance invariance (viz., makespan) and reproducibility.


It is worthwhile to define three regimes of ensemble execution
relative to resources and workload (tasks ready to run):
(1) there are inadequate resources to run the entire workload,
(2) there are adequate resources available to execute
the workload, and
(3) there are excessive (more than adequate) resources available
to execute the workload.
Understanding that the workload amount at any point in the
ensemble computation will vary, without loss of generality,
we can characterize the regimes.
In (1), the appropriate and optimal subset of tasks
will have to be selected and ordered to complete the workload.
That decision is non-trivial and can involve other criteria
than task performance per se. While tasks in a workload set
are independent, some might be determined to be of higher
priority.
In (3), the correct subset of
resources have to be selected, and the rest possibly released
to save cost.
In (2), the mapping of tasks to resources (which assumes
alternative task configurations) has to be optimal.
In all regimes, we are dealing with reasoning about the
workload performance concerning the collective.

Even if we knew the expected performance of each
task instance (for possible configurations and resource assignment), the scheduling
problem is difficult \textit{a priori}.
Allowing for even a tiny
variation in any task's performance makes finding the
``optimal'' schedule significantly harder. A distribution
of solutions will very likely be required.

Knowing whether a task's execution will be reproducible does little to make
the problem tractable.
% \jhanote{Allen: Something is missing in the previous
% sentence, but not sure what? Easier? Simpler? Tractable?}
If we forget about whether
task performance is reproducible, how should we define ``reproducibility'' in
the context of ensembles? One possible way to approach this is to simplify the
focus of the problem of scheduling the \textit{next} task. Indeed, given an
executing subset of workload tasks, the ensemble runtime system must
a) decide which task to execute next, b) select/allocate free
resources to that task, and c) configure the task appropriately.
Thus, the problem is reduced to deciding on the next task
and its execution.

It is not to say that the problem is now easy. If we had any
information about the performance of the remaining tasks,
that might be beneficial, but we have to assume it
will have performance variability. We may also need to consider non-stationary distributions from which individual task performance is drawn.
Having no knowledge of expected performance is
equivalent to high variability. Once a task begins, its
performance is determined by its execution. The workload performance as a collective will be determined by the
\textit{next} task assignment, task by task.
Interestingly, at those points extra information will
be available about which task(s) finished and how
resource availability may have changed as a result.
Furthermore, it is possible to gain further information
and insight into how well individual tasks are performing
by employing support for observation and monitoring
in the ensemble system.

In one sense, then, we could reason about ensemble reproducibility concerning
whether the same decision would be made about scheduling the next task if the
circumstances were the same in different ensemble executions, for every
ensemble task. Unfortunately, this reasoning falls on its face since any task
performance variation has the potential to make each ensemble execution
different. If, instead, we recast reproducibility as making ``locally
optimal''scheduling decisions, there is more consistency across multiple runs
of an ensemble computation that we can imagine.

Carrying this further, if we rationalize ensemble
computing concerning its potential for massive
makespan, we could imagine that its performance will
begin to conform to the \textit{Law of Large Numbers}.
That is, the greater the ``span'' of tasks off the critical
path, the less impact variations among those tasks will have
acute effects, even if they are scheduled differently.
That is rationally sound but likely difficult to actually
prove experimentally.

Lastly, although we have downplayed adaptability in this
paper, the institution of an observation and monitoring
framework would allow not only increased performance awareness
to better inform future scheduling decisions, but also
enable detection of performance anomalies when they arise,
allowing corrective actions, however possible. The situational
awareness of performance state coupled with in situ analytics
and dynamic response to problematic behavior will make
observation, monitoring, and adaptive control critical for
harnessing reproducibility in ensemble computing.

\begin{comment}

- Collective peformance and invariance
- Stationary versus non-stationary distributions
- Drawn from the same distribution, or not? KS



\admnote{This is as far as I got before my brain juice ran out.}

\begin{inparaenum}[1)]

% \item Performance is also drawn from a distribution, not a single value. 

% \item Whether that distribution is stationary or non-stationary is open question, and makes determining whether perf. is dynamic variable.

\item Given perf. distribution, distinguish between reproducible, variable and perf. portable

\item Ensemble execution conform Law of Large Numbers. Individual performance
might be statistically defined, but collective performance can be/is a
well-defined measure -- both at an instant of time, as well as over a window
of time.

\item Performance variability has implications when there are dependencies to resolve.

\item Three regimes: (1) Inadequate resource to run the full workload; (2)
Adequate resources are available to execute the workload, and (3) More than
adequate resources to execute the workload.  In (1) the appropriate and
optimal subset of tasks have to be selected. In (3) the right subset of
resources have to be selected. In (2) the mapping of tasks to resources has to
be optimal.

\item Discuss implications when we have adaptive execution, 
i.e., the challenges from the loss of performance reproducibility will only be
extenuated with adaptive applications and execution.

\item Unambiguously discerning and establishing factors responsible for performance
variability of tasks will require online task introspection, real-time global
and local execution environment awareness, and adaptive execution runtime
systems.


\item Online monitoring is necessary as a source of information to make
dynamic runtime decisions: task placement, scheduling, etc., and as a way to
respond to performance variability. The interest in dynamic runtime decisions
requires continuous performance monitoring of workload tasks, utilization of
resources, and ensemble system hardware and software layers. More significant
is the processing of the observed information with in situ analytics for
generating low-latency performance results for feedback to policy-driven
ensemble decision control. In general, the scalability of the observation,
monitoring, and analytics framework is critical for determining the degree of
dynamic awareness in the ensemble workload system and the latency of adaptive
response. Clearly, there is a symbiotic relationship between how well
many-task workload can be managed to most effectively utilize the HPC
resources and the timely processing of online information.



\end{inparaenum}

\end{comment}

==> discussion.tex <==
%!TEX root = ./paper.tex

\section{Discussion}

Before proceeding further down the path of performance reproducibility
in ensemble computations, it is beneficial to reflect on
performance variation assumptions of an HPC application.
It is generally expected that a deterministic application code will
exhibit minor, if any, relevant variation in its performance if it is
run in the same configuration on the same machine. It is this
expectation that forms the basis for HPC performance optimization where
inefficiencies can be reliably identified and improvements made.
That said, several exogenous factors can lead to
performance variation, including differences in processor clock rates,
contention with other running codes, operating system interference,
and more. Endogenous to an application, there can be non-determinism
inherent in its execution and fine sensitivities to memory and network
operation.

Nevertheless, it is reasonable to maintain the expectation of
minor performance variation in HPC applications; otherwise, our
performance optimization methodology breaks down. It might be
even assumed possible to characterize any variability within the
context of the application code, in order to determine bounds
and vulnerabilities. With this in mind, performance variation
for an HPC application can be generally regarded as a distribution
around expected performance value, one that very well might be
able to be reproduced.

However, ensemble execution is a different matter. All 
factors for performance variation of a single HPC application are
still valid for ensemble tasks. Instead of a single code, the variability analysis is compounded by the multiplicity of tasks.
In addition, it is essential to realize that how a task is
configured at the time of its execution and the resources assigned
are not necessarily fixed. The same task might be run in
a variety of configurations during the lifetime of the ensemble
computation. It is not the optimization of an individual task
under a particular configuration that matters. Instead, task performance
naturally has a much fuller distribution because it covers a
potentially broader set of options that the ensemble runtime system
has to choose from during task scheduling.

What implications does this have on performance reproducibility in ensemble computations?
Are we asking for individual task performance
to be reproducible, and by extrapolation, thinking the ensemble's performance should then be reproducible?
Given that an ensemble workflow
maintains task dependencies, does this imply that reproducibility will require invariance in task execution ordering from one ensemble run to the next?

We contend that the focus of reproducibility should not be on whether
an individual task's performance is reproducible in ensemble computation.
When a task is ready to run, it will then be scheduled and
configured according to the resources allocated. If the task is run
again at another point in the workflow, it might be configured
differently and with different resources. It makes little sense to
compare the two task executions if they are configured differently --
a 4-node MPI+OpenMP task with 32 CPU threads per node will behave
very differently from a 1-process instantiation of the task with 4 GPUs.
Here performance variation stares the ensemble scheduler directly
in the face.
Furthermore, decisions regarding resource assignment might have
less to do with optimal task performance than with dynamic resource
availability and collective utilization of ensemble resources.

It is worthwhile to define three regimes of ensemble execution
relative to resources and workload (tasks ready to run):
(1) there are inadequate resources to run the entire workload,
(2) there are adequate resources available to execute
the workload, and
(3) there are excessive (more than adequate) resources available
to execute the workload.
Understanding that the workload amount at any point in the
ensemble computation will vary, without loss of generality,
we can characterize the regimes.
In (1), the appropriate and optimal subset of tasks
will have to be selected and ordered to complete the workload.
That decision is non-trivial and can involve other criteria
than task performance per se. While tasks in a workload set
are independent, some might be determined to be of higher
priority.
In (3), the correct subset of
resources have to be selected, and the rest possibly released
to save cost.
In (2), the mapping of tasks to resources (which assumes
alternative task configurations) has to be optimal.
In all regimes, we are dealing with reasoning about the
workload performance concerning the collective.

Even if we knew the expected performance of each
task instance (for possible configurations and resource assignment), the scheduling
problem is difficult \textit{a priori}.
Allowing for even a tiny
variation in any task's performance makes finding the
``optimal'' schedule significantly harder. A distribution
of solutions will very likely be required.

Knowing whether a task's execution will be reproducible does little to make
the problem tractable.
% \jhanote{Allen: Something is missing in the previous
% sentence, but not sure what? Easier? Simpler? Tractable?}
If we forget about whether
task performance is reproducible, how should we define ``reproducibility'' in
the context of ensembles? One possible way to approach this is to simplify the
focus of the problem of scheduling the \textit{next} task. Indeed, given an
executing subset of workload tasks, the ensemble runtime system must
a) decide which task to execute next, b) select/allocate free
resources to that task, and c) configure the task appropriately.
Thus, the problem is reduced to deciding on the next task
and its execution.

It is not to say that the problem is now easy. If we had any
information about the performance of the remaining tasks,
that might be beneficial, but we have to assume it
will have performance variability.
Having no knowledge of expected performance is
equivalent to high variability. Once a task begins, its
performance is determined by its execution. The workload performance as a collective will be determined by the
\textit{next} task assignment, task by task.
Interestingly, at those points extra information will
be available about which task(s) finished and how
resource availability may have changed as a result.
Furthermore, it is possible to gain further information
and insight into how well individual tasks are performing
by employing support for observation and monitoring
in the ensemble system.

In one sense, then, we could reason about ensemble reproducibility concerning
whether the same decision would be made about scheduling the next task if the
circumstances were the same in different ensemble executions, for every
ensemble task. Unfortunately, this reasoning falls on its face since any task
performance variation has the potential to make each ensemble execution
different. If, instead, we recast reproducibility as making ``locally
optimal''scheduling decisions, there is more consistency across multiple runs
of an ensemble computation that we can imagine.

Carrying this further, if we rationalize ensemble
computing concerning its potential for massive
work-span, we could imagine that its performance will
begin to conform to the \textit{Law of Large Numbers}.
That is, the greater the ``span'' of tasks off the critical
path, the less impact variations among those tasks will have
acute effects, even if they are scheduled differently.
That is rationally sound but likely difficult to actually
prove experimentally.

Lastly, although we have downplayed adaptability in this
paper, the institution of an observation and monitoring
framework would allow not only increased performance awareness
to better inform future scheduling decisions, but also
enable detection of performance anomalies when they arise,
allowing corrective actions, however possible. The situational
awareness of performance state coupled with in situ analytics
and dynamic response to problematic behavior will make
observation, monitoring, and adaptive control critical for
harnessing reproducibility in ensemble computing.

\begin{comment}

- Stationary versus non-stationary distributions
- Drawn from the same distribution, or not? KS



\admnote{This is as far as I got before my brain juice ran out.}

\begin{inparaenum}[1)]

% \item Performance is also drawn from a distribution, not a single value. 

% \item Whether that distribution is stationary or non-stationary is open question, and makes determining whether perf. is dynamic variable.

\item Given perf. distribution, distinguish between reproducible, variable and perf. portable

\item Ensemble execution conform Law of Large Numbers. Individual performance
might be statistically defined, but collective performance can be/is a
well-defined measure -- both at an instant of time, as well as over a window
of time.

\item Performance variability has implications when there are dependencies to resolve.

\item Three regimes: (1) Inadequate resource to run the full workload; (2)
Adequate resources are available to execute the workload, and (3) More than
adequate resources to execute the workload.  In (1) the appropriate and
optimal subset of tasks have to be selected. In (3) the right subset of
resources have to be selected. In (2) the mapping of tasks to resources has to
be optimal.

\item Discuss implications when we have adaptive execution, 
i.e., the challenges from the loss of performance reproducibility will only be
extenuated with adaptive applications and execution.

\item Unambiguously discerning and establishing factors responsible for performance
variability of tasks will require online task introspection, real-time global
and local execution environment awareness, and adaptive execution runtime
systems.


\item Online monitoring is necessary as a source of information to make
dynamic runtime decisions: task placement, scheduling, etc., and as a way to
respond to performance variability. The interest in dynamic runtime decisions
requires continuous performance monitoring of workload tasks, utilization of
resources, and ensemble system hardware and software layers. More significant
is the processing of the observed information with in situ analytics for
generating low-latency performance results for feedback to policy-driven
ensemble decision control. In general, the scalability of the observation,
monitoring, and analytics framework is critical for determining the degree of
dynamic awareness in the ensemble workload system and the latency of adaptive
response. Clearly, there is a symbiotic relationship between how well
many-task workload can be managed to most effectively utilize the HPC
resources and the timely processing of online information.



\end{inparaenum}

\end{comment}

==> experience.tex <==
%!TEX root = ./paper.tex


\section{Experience}
